Crowdsourcing Diverse Paraphrases for Training Task-oriented Bots

A prominent approach to build datasets for training task-oriented bots is crowd-based paraphrasing. Current approaches, however, assume the crowd would naturally provide diverse paraphrases or focus only on lexical diversity. In this WiP we addressed an overlooked aspect of diversity, introducing an approach for guiding the crowdsourcing process towards paraphrases that are syntactically diverse.

==> HCOMP 2021 WiP - diversity/approach.tex <==


\vspace{-5pt}
\section{Crowdsourcing Diverse Paraphrases}


Figure \ref{fig:approach} depicts our approach and where it sits in an iterative and multi-stage pipeline for crowd-based paraphrasing based on prior art \cite{DBLP:conf/lrec/NegriMMGB12,kang-etal-2018-data,DBLP:conf/naacl/LarsonMLKHLHTM19}. 
%
% In this pipeline, a typical round $r$ of data collection (black arrows) takes an input set $X$ of seed utterances and runs it through paraphrase generation and validation steps.
%
In this pipeline, a typical round $r$ of data collection (black arrows) takes as input a dataset of seeds utterances $X$ and a curated collection of paraphrases $Y$ (initially, $Y$ can be empty).
%
The crowdsourcing task in the \textit{paraphrase generation} step asks a worker to provide a set of $n$ paraphrases $y_j$ for an utterance $x$. 
% The resulting collection of unverified paraphrases $\bar{Y}$ is fed to the \textit{paraphrase validation} step, where another crowd helps to identify the correct paraphrases that constitute the curated collection $Y$.
The resulting collection of unverified paraphrases $\bar{Y}$ is fed to the \textit{paraphrase validation} step, where another crowd helps to check for correctness. The correct paraphrases are then appended to the collection of curated paraphrases $Y$.
%
The \textit{seed selection} step updates (or fully replaces) the seeds in $X$ by sampling from the correct paraphrases to create the set of seeds for the next round.


Our approach assumes an initial ($X$, $Y$) as input and aims to steer the crowd towards specific \textit{patterns} or encourage workers to contribute novel syntactic variations to the input dataset. 
%Towards these goals, 
For these goals, we introduce a pattern selection step and propose novel prompts for paraphrase generation.
%
% Following \cite{DBLP:conf/naacl/IyyerWGZ18}, we use \textit{parse templates} (or \textit{patterns} for short) to capture and control syntax, where a \textit{pattern} is defined as the top two levels of a constituency parse tree (this depth mostly has clause/phrase level nodes, making syntax comparisons less strict but still effective).

%\subsubsection{Pattern selection}
\noindent\textbf{Pattern selection.}
% This work focuses on paraphrase generation (in red). 
%
% Following \cite{DBLP:conf/naacl/IyyerWGZ18}, we use \textit{parse templates} (or \textit{patterns} for short) to capture and control syntax, where a \textit{pattern} is defined as the top two levels of a constituency parse tree (this depth mostly has clause/phrase level nodes, making syntax comparisons less strict but still effective).
%
To capture and control syntax, we follow \cite{DBLP:conf/naacl/IyyerWGZ18} and define a pattern as the top two levels of a constituency parse tree (this depth mostly has clause/phrase level nodes, making syntax comparisons less strict but still effective).
%
% Our approach assumes an initial $X$ and $Y$ as input and aims to steer the crowd towards specific syntax or encourage workers to contribute novel syntactic variations to the input dataset.
%
The pattern selection step thus analyzes the paraphrases in $Y$ and identifies \textit{target patterns} to support the paraphrase generation step towards these goals.

% An important decision here is how we identify target patterns. 
% \textit{How do we identify target patterns?}
\textit{How to identify target patterns?}
For example, we may choose the $k$ least-frequent patterns in $Y$ as targets, or the $k$ most-frequent ones, any choice informing the generation step differently.
%
% Any of these choices inform the generation step differently. 
% The bottom-k patterns may be used to encourage workers to provide paraphrases matching any of the target patterns to collectively provide more balanced paraphrase structures.
Bottom-k patterns may be used to guide workers to provide paraphrases matching any target pattern to collectively contribute more balanced syntax.
While the top-k may be used as ``taboo'' to avoid frequent syntax.
% (i.e., to avoid paraphrases matching the target patterns).



% less-frequent.. encourage, steer
% most-frequent.. prevent/discourage


%(seeds utterances and curated paraphrases, respectively). 
% For each supported intent, the \textit{pattern selection} step defines as \textit{target patterns} the $k$ least-frequent patterns based on the paraphrases in $Y$.
%% "inspired by any of" vs "matching any of"








%\subsubsection{Paraphrase generation}
\noindent\textbf{Paraphrase generation.}
% While it is relatively straightforward to craft prompts for lexical variations (e.g., suggesting/forbidding words), it is not the case for syntactic variations, as patterns directly are not informative for non-experts.
Prompts can easily include words and ask workers to avoid/incorporate them in their paraphrases. 
%
This is not straightforward for patterns, as patterns directly are not informative for non-experts.


% \textit{How can the prompts leverage target patterns to steer towards (or encourage novel) syntactic variations?}
\textit{How can the prompts leverage target patterns to steer towards (or encourage novel) syntax?}
% 
To achieve these goals, this work proposes prompts that 1) impose constraints or 2) give recommendations, both by showing example words or paraphrases sampled from target patterns. 
% The prompts' goal defines what the target patterns represent.
% For example, sampled paraphrases/words can come from the bottom-k patterns.
% For example, target patterns could be the least frequent patterns in $Y$.
%
% Here, the prompts may include example paraphrases and ask workers to use one example as a reference and contribute paraphrases by just introducing lexical variations to the selected example (constraining workers to a specific syntax and compensating for less frequent syntax in $Y$).
%For example, if we set target patterns to the least frequent patterns in $Y$, the prompts may include example paraphrases and ask workers to use one example as a reference and contribute paraphrases by just introducing lexical variations to the selected example (constraining workers to a specific syntax and compensating for less frequent syntax in $Y$).
%
%The prompts, alternatively, may use the example paraphrases/words as recommendations to inspire workers and encourage them to contribute novel (or ``unseen'') patterns.
%
The specific goal shapes the prompt and what the target patterns represent.
%
For example, if we want to steer the crowd towards uncommon syntax, we can set target patterns to the least frequent patterns in $Y$. The prompts can then show example paraphrases sampled from these patterns and ask workers to contribute paraphrases matching a pattern in any example (i.e., constraining workers to a specific syntax and compensating for less frequent syntax in $Y$).
%
% The prompts, alternatively, may use example paraphrases/words as recommendations to inspire workers and encourage them to contribute novel (or ``unseen'') patterns.
Alternatively, we may aim for novel syntax, so the prompts may use example paraphrases/words as recommendations to inspire workers and encourage them to contribute novel (or ``unseen'') patterns. 




% The \textit{paraphrase generation} then prompts each worker for paraphrases with a pattern different than a seed $x$. It does so by 1) giving recommendations or 2) imposing constraints, both via example paraphrases/words sampled from the target patterns (as patterns directly are not informative for non-experts).
%
% Recommendations aim to obtain novel (or ``unseen'') patterns while constraining seeks to balance the number of paraphrases per pattern in the dataset.


% 
%Example paraphrases/words recommendations aim to obtain novel patterns not present in the input dataset while constraining seeks to balance the number of paraphrases associated with each pattern.





%The \textit{paraphrase generation} then prompts each worker to generate paraphrases with a pattern different than a seed $x$, and it does so by 1) constraining workers to produce paraphrases matching any of the target patterns, or 2) asking them to use the target patterns as inspiration and contribute paraphrases with a pattern similar to any target pattern or novel paraphrase with a novel syntax.

% The \textit{paraphrase generation} then prompts each worker to generate paraphrases with a pattern different than a seed $x$, and it does so by giving recommendations or imposing constraints based on the target patterns (as we can not show target patterns directly). Example words or paraphrases 




% Workers are then asked to contribute paraphrases with patterns different than the seed utterances
% We then prompt workers for paraphrases with a pattern deviating from the seed



% The intuition behind our approach is simple: we ask for paraphrases with a pattern different than the input utterance, and we obtain such paraphrases by showing example utterances for workers to use as inspiration, leveraging the inherent priming effect in paraphrasing tasks to our advantage \cite{DBLP:conf/acl/JiangKL17}. 
% %
% Therefore, it is critical what strategy we use to select these examples.
% %
% For each batch/round of paraphrasing, we just compute the distribution of patterns for each supported intent and select the $k$ least-frequent elements as our \textit{target patterns}. The examples shown to workers are then sampled from the target patterns.








% The structure of the task interface and the instructions are prescribed by the template style, while the prompt defines the scope (i.e., the intent), concrete descriptions, and examples shown to guide workers in solving the task.
% %
% For example, in a paraphrasing task, the template style may define how the instructions are framed and how many paraphrases the worker should provide. The prompt then represents the seed utterance shown to the workers for paraphrasing.




% We formulate the problem in the context of crowdsourcing utterance paraphrase sets for training task-oriented bots for the \textit{intent recognition} task, i.e., the ability of bots  to interpret natural language user requests. 
% Given an input utterance $x$, we can define paraphrasing as the problem of generating a set of $n$ utterance paraphrases $Y=\{y_1,y_2, ..., y_n\}$ so that each $y \in Y$ is generated by introducing \textit{variations} of $x$ while keeping the same meaning \cite{cao2020divgan}.
% %
% While the quality of paraphrasing is a much more involved concept \cite{DBLP:journals/internet/Yaghoub-Zadeh-Fard20}, in this work we focus on  \textit{diversity}, as the breath and variety of paraphrases in the resulting corpus.




% Paraphrasing techniques generally rely on approaches that aim at introducing \textit{lexical} and \textit{syntactic} variations. Lexical variations refer to changes that affect individual words, such as substituting words by their synonyms \cite{parikh2020automated}. Syntactic variations, instead, refer to changes in sentence or phrasal structure, such as transforming the grammatical structure of a sentence \cite{huang2021generating}. 
% While the development of techniques to introduce such lexical and syntactic variations is the focus of ongoing work in automatic paraphrasing, they are currently greatly under-explored in the crowdsourcing community.






%%The quality of these techniques is commonly measured\footnote{Quality aspects such as fluidity, grammatical correctness, and other dimensions explored especially in the context of crowdsourcing \cite{yaghoub2020user}, are not addressed in this work} in terms of the semantic \textit{relevance}, denoting the extent to which the output paraphrases are similar in meaning to the input utterance,  and \textit{diversity}, as the breath and variety of paraphrases in the resulting corpus \cite{yaghoub2020user}. 


% The intuition behind our approach is simple: we ask for paraphrases with a pattern different than the input utterance, and we obtain such paraphrases by showing example utterances for workers to use as inspiration, leveraging the inherent priming effect in paraphrasing tasks to our advantage \cite{DBLP:conf/acl/JiangKL17}. 
% %
% Therefore, it is critical what strategy we use to select these examples.
% %
% For each batch/round of paraphrasing, we just compute the distribution of patterns for each supported intent and select the $k$ least-frequent elements as our \textit{target patterns}. The examples shown to workers are then sampled from the target patterns.




% Preliminary results indicate that our proposed approach produces more diverse data than existing data collection methods and better results in a downstream task: intent detection.
% %
% The prompt proposed in this work can easily be coupled with existing techniques. For example, by including word suggestions \cite{DBLP:conf/iui/Yaghoub-Zadeh-Fard20}, we can achieve further gains in terms of diversity and intent detection performance.



